IoTRepair: Systematically Addressing Device Faults in Commodity IoT (Extended Paper)

IoT devices are decentralized and deployed in un-stable environments, which causes them to be prone to various kinds of faults, such as device failure and network disruption. Yet, current IoT platforms require programmers to handle faults manually, a complex and error-prone task. In this paper, we present IoTRepair, a fault-handling system for IoT that (1)integrates a fault identification module to track faulty devices,(2) provides a library of fault-handling functions for effectively handling different fault types, (3) provides a fault handler on top of the library for autonomous IoT fault handling, with user and developer configuration as input. Through an evaluation in a simulated lab environment and with various fault injectio nmethods,IoTRepair is compared with current fault-handling solutions. The fault handler reduces the incorrect states on average 50.01%, which corresponds to less unsafe and insecure device states. Overall, through a systematic design of an IoT fault handler, we provide users flexibility and convenience in handling complex IoT fault handling, allowing safer IoT environments.

==> algorithms/rollback.tex <==
\begin{algorithm}[t!]
    \DontPrintSemicolon
    \footnotesize
    \setstretch{1}
	\SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
	\DontPrintSemicolon
	\SetNoFillComment % <---------------------------
	\Input{The $ID$ of the device that triggered this rollback}
	\Output{Success or Failure}
	$\mathit{targetCriteria} \gets \mbox{(systemState,fail-safe states,rollbackType)}$ \;
    $bestMatch \gets \emptyset$
    \BlankLine
    \ForEach{$\mathit{checkpoint}$ \normalfont{in} $\mathit{Checkpoints}$}{
        \If{$\mathit{checkpoint}$ \normalfont{meets} $\mathit{targetCriteria}$ \normalfont{better than} $\mathit{bestMatch}$}{$\mathit{bestMatch} \gets \mathit{checkpoint}$}
    }
    \If{$\mathit{bestMatch}$ \normalfont{equals} $\emptyset$}{$\mbox{return}$ $\mbox{Failure}$}
    \ForEach{$\mathit{device}$ \normalfont{in} $\mathit{bestMatch}$}{
        \If{$\mathit{device}$ \normalfont{is a faulty actuator and requires a state change}}{ $\mbox{return}$ $\mbox{Failure}$}
    }
    \ForEach{$\mathit{device}$ \normalfont{in} $\mathit{bestMatch}$}{
        \If{$\mathit{device}$ \normalfont{is actuator and requires a state change}}{ $\mbox{actuate device.id to device.state}$}
    }
    \ForEach{$\mathit{deviceCheckpoint}$ \normalfont{in} $\mathit{bestMatch}$}{
        \If{$\mathit{matchingDevice}$ \normalfont{is a faulty sensor}}{$\mbox{matchingDevice.state} \gets \mbox{deviceCheckpoint.state}$}
    }
    $\mbox{return}$ $\mbox{Success}$
    \caption{Algorithm For Rollback\label{alg:Rollback}}
\end{algorithm}

%% \gang{When you put words into the latex math mode, we need to surround it by mbox or mathit; otherwise, the spacing would look funny. Typically, you put variables in mathit and non-variables (e.g., keywords) in mbox. For example, write $\mbox{Success}$ and $\mathit{device}$. Please fix the above figure and others.}



==> algorithms/transaction.tex <==
\begin{algorithm}[t!]
    \DontPrintSemicolon
    \footnotesize
    \setstretch{1}
	\SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
	\DontPrintSemicolon
	\SetNoFillComment % <---------------------------
	\Input{An $\mathit{ActuationList}$ of ($\mathit{ActuatorID,ActuationValue}$) tuples}
	\Output{Success or Failure return code}
	$ \mathit{undoLog}s \gets \emptyset$
    \BlankLine
    \ForEach{$\mathit{tuple}$ \normalfont{in} $\mathit{ActuationList}$}{
        $\mathit{originalValue}$ $\gets$ $\mathrm{getDeviceState}$($\mathit{tuple}$[0])\;
        \If{actuate($\mathit{tuple}$[0],$\mathit{tuple}$[1]) \normalfont{returns} Failure}{
            \ForEach{$\mathit{actuatio}n$ \normalfont{in} $\mathit{undoLog}$}{
                actuate(actuation[0], actuation[1])
            }
            $\mbox{return}$ $\mbox{Failure}$
        }
        $\mathit{undoLog}$.append($\mathit{tuple}$[0], $\mathit{originalValue}$)
    }
    $\mbox{return}$ $\mbox{Success}$
    \caption{Algorithm For Transaction\label{alg:Transaction}}
\end{algorithm}


==> tables/applicationsAbridged.tex <==
\begin{table*}[th!]
\def\arraystretch{1}
\setlength{\tabcolsep}{1.1pt}
\resizebox{\textwidth}{!}
{%
\begin{threeparttable}[b]
\begin{tabular}{|l|l|l|c|}
\hline
\textbf{ID} & \textbf{App Name} & \textbf{Description}  \\ \hline \hline
\texttt{App1} & Motion-Activated-Lights & When motion detected, turn on lights. Turn off lights when motion not active. \\ \hline
\texttt{App2} & Smoke-Alarm & When smoke is detected sound alarm and unlock doors. When no smoke is detected turn off alarm.  \\ \hline
\texttt{App3} & Temperature-Control & Keep temperature between 70-80 degrees (\degree F) by turning heater and air conditioner on and off  \\ \hline
\texttt{App4} & Water-Leak-Detector & When leak is detected sound alarm and close water valve. When no leak is detected turn off alarm and open water valve.  \\ \hline
\texttt{App5} & Welcome-Home & When the user arrives home, unlock doors and turn on coffee machine  \\ \hline
\texttt{App6} & Secure-Patio & When user is not present and contact is detected, send text message to user \\ \hline
\texttt{App7} & Energy-Saver & If window is open and either heater or air conditioner is on, close window. \\ \hline
\texttt{App8} & Secure-Home & when user is not present home, lock doors and close windows. \\ \hline
\texttt{App9} & Intruder-Detector & When user is not present home and motion is detected, send text message to user \\ \hline
\texttt{App10} & Alarm-Safety & When alarm is activated, turn on lights \\ \hline
\texttt{App11} & Morning-Air & Open windows and close windows at specific times \\ \hline
\end{tabular}
\end{threeparttable}
}
\caption{IoT apps and their descritpions, developed to evaluate \sysname{}.}
\label{table:applications}
\end{table*}

